Memory-assisted prompt editing to improve GPT-3 after deployment

Large LMs such as GPT-3 are powerful, but can commit mistakes that are obvious to humans. For example, GPT-3 would mistakenly interpret "What word is similar to good?" to mean a homophone, while the user intended a synonym. Our goal is to effectively correct such errors via user interactions with the system but without retraining, which will be prohibitively costly. We pair GPT-3 with a growing memory of recorded cases where the model misunderstood the user's intents, along with user feedback for clarification. Such a memory allows our system to produce enhanced prompts for any new query based on the user feedback for error correction on similar cases in the past. On four tasks (two lexical tasks, two advanced ethical reasoning tasks), we show how a (simulated) user can interactively teach a deployed GPT-3, substantially increasing its accuracy over the queries with different kinds of misunderstandings by the GPT-3. Our approach is a step towards the low-cost utility enhancement for very large pre-trained LMs. Code, data, and instructions to implement MEMPROMPT for a new task at https://www.memprompt.com/.

==> sections/faq.tex <==
\section{FAQ}
In this section, we attempt to clarify the contributions of our work and how it relates to other related work.

\begin{enumerate}
    \item \textbf{How is this work related to prompt tuning?}
    Prompt tuning, or the idea of prepending an input with an informative prefix has gained a lot of attention. Our work is closely related to prompt-tuning, and introduces a new kind of prompt (feedback prompt). This allows us to train systems that can react to feedback given by the users.
    \item \textbf{How is this related to instruction tuning?}
    Instruction-prompting refers to phrasing the question posed we Our work is closely related to instruction tuning, and takes it one step ahead. In addition to having the instruction in the input, we also have the understanding of the task instruction in the output. This helps the person in giving feedback even when they are not clear about the task.
    \item \textbf{How is this related to few-shot prompting?}
    Our work is closely related to few-shot prompting. Specifically, we present a way to dynamically update the few-shot prompt using a memory.
    \item \textbf{The dataset is too small?}
    \item Why cannot the prompt be grown as more examples come in?
\end{enumerate}

==> sections/figures/delphi/instracc.tex <==
\begin{figure}
\centering
    \begin{tikzpicture}
        \begin{axis}[
        	xlabel=Time,
        	ylabel=Instruction Accuracy, %Performance,
        	width=1\columnwidth,height=7cm,
        	axis background/.style={fill=white},
            legend style={at={(0.73,0.15)},anchor=west}]
        \addplot[color=red,mark=diamond, smooth] coordinates {
(0, 19)
(100, 25)
(200, 27)
(300, 27)
(400, 28)
(500, 30)
(600, 29)
(700, 30)
(800, 30)
(900, 31)
        };
        \addplot[color=blue,mark=pentagon, smooth] coordinates {
(0, 21)
(100, 19)
(200, 24)
(300, 25)
(400, 26)
(500, 28)
(600, 29)
(700, 30)
(800, 31)
(900, 31)
        };
        \addplot[color=orange,mark=square, smooth] coordinates {
(0, 10)
(100, 17)
(200, 22)
(300, 25)
(400, 25)
(500, 24)
(600, 23)
(700, 25)
(800, 26)
(900, 27)
};
        \legend{1.0, 0.5, 0.15}
        \end{axis}
        \end{tikzpicture}
    \caption{\ertcat: Instruction accuracy sharply increases with a larger clarification probability. This shows that \ours responds to feedback.}
    \label{fig:delphiinstraccuracy}
\end{figure}


==> sections/figures/delphi/labelacc.tex <==
\begin{figure}
\centering
    \begin{tikzpicture}
        \begin{axis}[
        	xlabel=Time,
        	ylabel=Label Accuracy, %Performance,
        	width=1.1\columnwidth,height=8cm,
        	axis background/.style={fill=white},
            legend style={at={(0.65,0.45)},anchor=west}]
        \addplot[color=green,mark=diamond,smooth] coordinates {
(0, 56)
(100, 53)
(200, 57)
(300, 58)
(400, 57)
(500, 58)
(600, 58)
(700, 58)
(800, 58)
(900, 58)
        };
        \addplot[color=red,mark=pentagon] coordinates {
(0, 48)
(100, 50)
(200, 53)
(300, 53)
(400, 53)
(500, 55)
(600, 55)
(700, 57)
(800, 57)
(900, 57)
        };
        \addplot[color=orange,mark=square, smooth] coordinates {
(0, 52)
(100, 49)
(200, 52)
(300, 53)
(400, 54)
(500, 53)
(600, 54)
(700, 55)
(800, 55)
(900, 56)
};
        \addplot[color=blue,mark=triangle, smooth] coordinates {
(0, 45)
(100, 48)
(200, 48)
(300, 48)
(400, 48)
(500, 48)
(600, 47)
(700, 46)
(800, 47)
(900, 46)
};
        \legend{1.0, 0.5, 0.15, \nomem}
        \end{axis}
        \end{tikzpicture}
    \caption{\ertcat: Label accuracy increases with time}
    \label{fig:delphicataccuracy}
\end{figure}


==> sections/method_old.tex <==
\section{Approach}
\label{sec:method}
In this section, we first present a general overview of our approach, followed by a specific instantiation of this general setup on a QA task.

\paragraph{Background: Few-shot prompting with \gptshort}  We focus on a general setup where given an input \quesm, a model is expected to generate an output \ansm. 
We use \gpt in few-shot prompting mode~\citep{Brown2020GPT3}, where a prompt \promptm consists of $k$ $(\ques, \ans)$ examples.
Each sample $(\ques, \ans)$ is concatenated as a string, and samples are separated by a special symbol \sepm to create the prompt $\prompt = \ques_1 . \ans_1 \sep \ques_2 . \ans_2 \ldots \sep \ques_k . \ans_k$.
% $$\prompt = [(\ques_i, \ra_i,  \ans_i)]_{i=1}^{k}\ \sep\ [(\ques_j, \fb_j, \ra_j, \ans_j)]_{j=1}^{k} $$
During inference, the user inputs a question $\ques_i$, and the model is fed $\prompt\ \sep\ \ques_i$ (\ie the question suffixed to the prompt) and is expected to generate the answer $\ans_i$.



% and its understanding of the instruction, $\ra = \textit{i am generating an synonym}$., and an understanding of the instruction in the input, \ram.
% and its understanding of the question $\ra_i$.
% For example, for a lexical question-answering task, given an input question $\ques = \textit{what is similar to fast?}$, the model generates the answer $\ans = \textit{quick}$.

\subsection{Memory enhanced \gptshort architecture}

We extend the above outlined few-shot prompting setup with a memory of errors.
We achieve this by slightly modifying the task to include model's understanding of the input, and by implementing a memory module that records past errors and retrieves relevant feedback for a given input.
We expand on these two components next.



\begin{figure}[!h]
\centering
    \includegraphics[scale=0.24]{sections/figures/architecture}
    \caption{Proposed architecture: (left) \gptshort does not account for user feedback. (right) \ours maintains a memory $\memory$ and searches for a key in $\memory$ with a similar intent as $x$ using \retm. The  combiner combines x and retrieved feedback which is then appended to the prompt for querying \gptshort. 
    % This allows \gptshort to better understand the user and generate the right answer. 
    The user can provide any feedback $f$ which gets written to $\memory$.}
    \label{fig:method}
\end{figure}

\paragraph{Generating model's understanding of intent} 
In most cases, the user may not know the correct output \ansm for a given \quesm, making it impossible to provide any feedback to the model after deployment.
However, the user might be able to give a feedback on model's understanding of the task, denoted as \ram.
Further, an incorrect understanding of the task can be expected to translate into an incorrect output in most cases, making \ram a suitable proxy for correctness of the model.
We exploit this insight to obtain useful feedback, \fbm, from the users.
This feedback, denoted as \fbm, is used to clarify the intended usage of the question to the model.

As a concrete example, consider a situation where the user asks for the antonym of a word $\ques = \textit{what is the opposite of fast?}$, and the model generates $\ans = \textit{quick}$ and $\ra = \textit{i am generating the something like fast}$.
Here, the user might give the model a feedback \fbm = \textit{when I ask for an opposite of something, I want an antonym}.
To enable the model to react to such feedback, we include a number of samples of the form \fbsample in the prompt, where the feedback $\fb$ is included with each question.
We call this prompt the \textit{feedback prompt}.

\paragraph{Memory of errors} 
Consider a case in which the user detects that model's understanding of the question \ram is incorrect and supplies a feedback \fbm.
The feedback might be relevant for other similar questions that the model might misunderstand.
To prevent the model from making repeated mistakes, we supplement the few-shot prompting workflow by using a memory of feedbacks \memorym.
We illustrate our method with an example below and in Figure~\ref{fig:method}.

Given an input \quesm, our method~(\ours) does not directly perform few-shot prompting.
Rather, it first queries the memory \memorym using a retriever \retm for a relevant feedback \fbm (\ie $\fb = \ret(\ques, \memory)$.
If such a feedback is found, it is attached to the input \quesm and the few-shot prompting is carried out using the feedback prompt.

Similarly, given model output $(\ques, \ra)$, the user may give a feedback on \ram with a probability $\Pr(\fb)$.
This feedback is recorded in the memory (\ie $\memory(\ques) = \fb$).

% We propose a method to enhance \gptshort with a memory of errors and feedback. The input x is a question, and output y is an answer and an explanaiton/understanding u of the model. A user can give feedback on a wrong u. This gets written to a memory. So the next time a user queries the same x or with a similar x, then we can apply the feedback given in a similar situation. The modules of this are show in Figure 3, overview shows there is M and g. There is a retrieval step from M.. and $x'_j = \Omega(M, g, x_j)$ . This is applied to the prompt.



\begin{figure}[!t]
\centering
    \includegraphics[scale=0.26]{sections/figures/task-memory.pdf}
    \caption{A sample of memory for the task of lexical question-answering. \niket{show query}}
    \label{fig:memsample}
\end{figure}


\subsection{A Proof of Concept Implementation}
\paragraph{Task}
In this work, we focus on lexical question-answering task, where the user can ask five different kinds of questions about a given word.
These include synonym, antonym, homonym, definition, and usage in a sentence.
We choose this task as each question can be asked in multiple ways~(\eg for synonym generation, the users might ask questions of the form \textit{what is like}, \textit{what has a similar sense}, \textit{what is akin to}, \textit{what is something like}, etc.)
Further, unlike long-form generation tasks, we can fit a large number of samples in the prompt, giving us a strong baseline that we can use to compare our approach with.
We use the feedback prompt with 10 examples of the task.
The prompt is included in Appendix~\secref{sec:actualprompt}~(Figure~\ref{fig:actualprompt}).
% As outlined above, given a question \quesm, a model is expected to generate an answer \ansm, and an understanding of the instruction in the question, \ram.
% For example, given a question $\ques = \textit{what is similar to fast?}$, the model generates the answer $\ans = \textit{quick}$.
% Additionally, the model generates its understanding of the instruction, $\ra = \textit{i am generating an synonym}$.
% Thus, each sample is for the form tuple \sample.



\paragraph{Implementation of \memorym } 
We implement a \memorym by using \quesm as the key and the corresponding feedback \fbm as value.
Given a question $\ques_i$, if the user detects that the model has misunderstood the question, they may provide a $\fb_i$ with probability \fprobi.
The feedback is stored in a memory \memorym, with $\ques_i$ as the key and $\fb_i$ as the value. 

For a subsequent question $\ques_j$, the retriever \retm (described below) checks if a similar question appears in memory.
If yes, then the corresponding feedback is attached with the question and fed to the model for generation.


For example, the model might misunderstand the question \textit{what is akin to fast ?} as one that requires antonyms. The user, by inspecting the \ram = \textit{i am generating the opposite of fast} might determine that the model has in fact misunderstood them, and give a feedback \textit{i wanted a synonym}, which is stored in \memorym.
If a similar question~(\eg \textit{what is akin to pretty ?}) is asked later by the same or a different user, the corresponding feedback~(\textit{i wanted a synonym}) is attached with the question to generate the correct answer.



Crucially, while the ability of the model to understand a question has not changed~(the model will continue to mistake akin as a query for antonym), feedback allows it to correct the behavior.
Note again that the model is able to reach to the feedback because of examples in the prompt that contain feedback.
Figure~\ref{fig:memsample} shows a small sample of the memory we have for this task.

\paragraph{Implementation of \retm} An incorrect feedback might cause the model to make a mistake where it would have gotten the correct answer without any feedback.
A good retriever is crucial to prevent such cases.
For more difficult use cases, example those involving structured generation, a retrieval that performs analogical reasoning with the input might be required.
In our setting, we use two different retrieval functions:
% If such a matching (similar) question $\ques_{m}$ is found, we attach the corresponding clarification $\fb_{m}$ to the query and feed $\prompt\ \sep\ \ques_j \ct \fb_{m}$ to the model. 
% Otherwise, we feed just the question to the model (\ie $\prompt\ \sep\ \ques_j$).
% We experiment with two different similarity functions $\texttt{sim}$, and use a threshold $\tau$ to ascertain similarity~(\ie $\texttt{sim}(\ques_{m}, \ques_j) > \tau$).

% \pete{That's important to mention in the paper too. Again, it's worth framing this as a kind of placeholder in the architecture, requiring future work to do this gating properly}
% \todo{context: mention that we avoid cases where the model would have gotten it right regardless by using a threshold, and mention that in the future the gating could be fancier (\eg we want a analogy based retrieval for proscript}
\noindent (1) Semantic similarity: the query is encoded using Sentence transformers~\citep{reimers-2019-sentence-bert}, and use cosine distance between the query $\ques_i$ and every key in the memory to find a matching key $\ques_m$. We use a threshold of 0.9.
    
\noindent (2) Lexical similarity: We also experiment with low-resource settings for which trained retrieval is not an option. In such cases, we rely on a number of heuristics to perform similarity matching between a given question and a question in the memory. The details are included in the Appendix~\secref{sec:simquestions}.



% \paragraph{Why does the model need to generate \ram?} A key insight of our method is that a user cannot provide feedback to the model on its output in general.
% Suppose a user poses a rephrased version of the antonym question $\ques = \textit{what is the opposite of good?}$.
% If the model generates $\textit{great}$ as the answer, the user may not know the right answer and may simply accept the incorrect answer.
% On the other hand, a model that additionally provides the user with its understanding $\ra = \textit{i am generating a synonym}$ allows the user to clarify what they actually wanted to ask (antonym) without knowing the right answer.
% In realistic settings, \ram is the only way of determining if the model understood the query, allowing for feedback that can be reused.






% * Task: Few-shot examples of the form X --> R, ans.
% * Additionally, we have examples of the form (X, clarification --> R, ans).
% * Input = [X --> R, ans] + [X, clarification --> R, ans]
% * Model gives two things as output (R, ans)
% * R is used by the user to provide a feedback to the model.
% * The feedback is recorded in a memory.
% * For the next input, 

% - Emphasize on simplicity

% - Give running example

%  -> What is the antonym of good? What is unlike good?
%  We add two examples:

% - (What is the antonym of good? -> \underline{You are asking for the antonym of good} \textit{The answer is bad})
 
% - (What is unlike good? | clarification when I want unlike, I really want an antonym -> \textit{You are asking for the antonym of good} \textit{The answer is bad})

% Notations:
% few shot examples -> list (qi -> ai, ri) + list (qj, fj -> aj, rj)
% ques -> q
% rationale -> r
% answer -> a
% feedback -> f
% memory (key, value) Mem(k,v)
% input prompt (x)
% output answer (y)

% % # High level introduction
% % # Notations
% % # Examples
% % # Diagram
% % # Memory (read and write)
% % # Retrieval
% % # Applying the feedback



==> sections/sections_archived/intro-v0.tex <==
\section{Introduction}

% \begin{enumerate}
%     \item Designing prompts that can adapt and personalize.
% Add multitasking with clarifications
%     \item Generating output that is amenable to feedback.
% Expose reasoning mechanism with the output/exposes internal beliefs
%     \item Preventing the model from making the same mistake twice. Use a simpler form of memory. This is an explicit memory (not soft memory)
% \end{enumerate}



% \gptshort a powerful model however, it is not immune to mistakes \citep{marcus_gpt3}.
\gptshort while powerful, is not immune to mistakes \citep{marcus_gpt3}.
The typical remedy of re-training the model with more data is not easy for these very large models, due to the prohibitive cost and infrastructure requirements. 
% \red{PC: Could drop next sentence}
% Moreover, such modifications might be explicitly disallowed by the distributors of the model.\footnote{\gpt (\textit{davinci}) cannot be fine-tuned using openai api currently without prior approval.}
In such cases, even if the users observe the model making a mistake repeatedly, there are no avenues to provide feedback to the model.
%, especially so, for an end user. 
Consider the example in Figure \ref{fig:running-example}, where a user performs a lexical task to find synonyms. Depending on the user's expertise, and dialect, the 
task may be expressed in various ways. The model performs well until it encounters a new dialect or a poorly worded task.

\begin{figure}[!t]
% \vspace{-4em}
\centerline{
\fbox{%
    \parbox{0.49\textwidth}{%
	\underline{Our memory enhanced GPT-3 implementation.}
% \vspace{2mm}
% \red{PC: I wouldn't use different font for `similar to' etc., it makes it look like it's specially flagged in the input to GPT3
% somehow}
\begin{des}
% \item[{\bf User:}] What is akin to slam?
% \item[{\bf \gptshort:}] I am generating a homonym: lamb.
% \item[{\bf User:}] By akin to, I mean a similar word.
% \item[{\bf \gptshort:}] Noted \textit{(writes to memory)}.
% \item[{\bf User:}] What is akin to wonderful?
% \item[{\bf \gptshort:}] I applied a past feedback \textit{akin to means a similar word}. I am generating a synonym: lovely.
\item[{\bf User:}] What word is similar to ‘good’?
\item[{\bf \gptshort:}] Generating a homonym: wood.
\item[{\bf User:}] "Similar to" means "with a similar meaning".
\item[{\bf \gptshort:}] Noted {\it [writes to memory]}
\item[{\bf User:}] What word is similar to 'surprised'?
\item[{\bf \gptshort:}] {\it [Retrieves and adds to prompt '"Similar to" means "with a similar meaning"']}. \\
        Generating a synonym: amazed.

\end{des}
    }%
}}
\caption{This paper enhances GPT-3 performance by looking up questions with a similar intent that received any user feedback. Our approach is simple because only the prompt needs to be updated with the retrieved relevant feedback, and no retraining is necessary.}
\label{fig:running-example}
\end{figure}

% \pete{I think you want to draw out an important insight/idea in the paper,
% namely to have GPT3 repeat its understanding of the user's intent, as 
% well as the answer itself.}
What happens if the user realizes that the model's understanding is not correct and wants to help fix it? Note that such a correction is feasible {\it even if the user does not know the answer to their question}, as they are critiquing the model's understanding of their intent rather the answers themselves. 
A recent approach called few-shot learning \cite{Brown2020GPT3} allows a user to supply a series of examples of the task that the model is supposed to perform. These examples are concatenated with the input to form a prompt. One could envision an approach to extend few-shot learning to append the user feedback ($\fb$) in the input prompt as a way of providing a signal to the model. However, such an envisioned approach would have several shortcomings. (1) the prompt must be repeatedly updated for the same example. (2) there is no mechanism to improve the performance over time. (3) the number of tokens in the prompt are limited.

We overcome these challenges by supplementing a prompt with a memory of feedbacks. We maintain a memory of user interactions as key-value pairs, where the key is a question context, and the value is a feedback that the model received. Given a new question, we check if the model has made a mistake on a similar question earlier, by querying the memory for a similar question and append the matching key's feedback to the question prompt. We prevent the model from making the same mistake twice. We assume that the model provides a window to its internal belief to allow critiquing e.g., by additionally generating an explanation, or an evidence of its understanding of the question. Thus, we allow users to provide $\fb$ on the model's understanding, offering a route for users to continually teach the machine about new topics. We show empirically that \ours is a valid solution to incorporate feedback, and achieves the best results on five lexical tasks by a large margin. 

\ours leverages the success of prompts to incorporate \fbm and our idea of memory draws inspiration from the theory of recursive reminding in psychology \cite{Jacoby2013}. The theory suggests that humans remember (in the episodic memory for an event) the context in which they made an error and the received correction. Humans think not only of the error but also of the surrounding context in which it was made and associate it with the correction. In line with this theory, we record the learner's~(model's) mistakes and the feedback from user in a learner's memory.

In summary, our main contribution is a simple approach to allow users to correct a deployed model's errors directly through interaction -- without retraining. We ground the benefits of our method empirically with simple proof-of-concept experiments. 

% In summary, we propose a novel mechanism to allow users to correct model errors directly through interaction -- without retraining.
% We achieve this by supplementing \gpt with a memory of errors and user feedback.
% Our simple proof-of-concept experiments show that a user can interactively teach \gptshort in this way, doubling its accuracy on basic lexical tasks (e.g., generate a synonym) where instructions are stated in different (sometimes misunderstood) ways.

% Inspired by the concept of memory from recursive reminding, we propose a simple approach to maintain a memory of user interactions as key-value pairs, where the key is a question that the model has incorrectly answered, and the value is a user feedback text applicable for this question. 
% Given a new question, we enhance \gptshort with this memory by retrieving relevant past feedback from the memory and appending it to the question. 
% We show empirically that a memory enhanced \gptshort is a valid solution to incorporating feedback in a model, and achieves the best results on five lexical tasks by a large margin. 





% Our approach is motivated by the following key insights:
% \squishlist
% \item If the model is wrong about a question, it will continue to be wrong unless it is retrained.
% \item In realistic settings, a user cannot provide a feedback on the output of the model, as the correct answer might be unknown to the user. However, it is more accessible for the user to provide a feedback on model's understanding of the question.
% \squishend








% \newpage
% \clearpage
% \begin{figure*}[!ht]
% \centering
%     \includegraphics[scale=0.30]{sections/figures/memprompt-method-baseline-memory-2-col.pdf}
%     \caption{Overview method option 2}
%     \label{fig:method}
% \end{figure*}

% \begin{figure*}[!ht]
% \centering
%     \includegraphics[scale=0.26]{sections/figures/memprompt-method-read-write-baseline-v2.pdf}
%     \caption{Overview method option 3}
%     \label{fig:method}
% \end{figure*}




% NT: temporarily commenting
% \corr{We design a very simple approach to provide feedback on the model's understanding, offering a route for users to continually teach the machine about new topics.}{We design a simple approach that allows users to provide a feedback on the model's understanding, offering a route for users to continually teach the machine about new topics.}
% \corr{We maintain a memory of user interactions, as key value pairs where the key is a rationale text and optionally the context text, and the value is a user feedback text applicable for this rationale.}{We maintain a memory of user interactions as key-value pairs, where the key is a question that the model has incorrectly answered, and the value is a user feedback text applicable for this question.}

% Given a new question, we enhance \gptshort with this memory by retrieving relevant past feedback from the memory and appending it to the question.
% We show empirically that a memory enhanced \gptshort is a valid solution to incorporating feedback in a model, and achieves the best results on five lexical tasks by a large margin.

% \am{realistically, it is impossible to give feedback on the answer: if the user already knows the answer, they will not be asking the model. However, a user can always correct the model on explanation.}
% \am{Key points: i) we allow feedback on model's understanding, ii) we are all about \textbf{no ft}: think OOV etc.}




